DynAlign: Unsupervised Dynamic Taxonomy Alignment for Cross-Domain Segmentation

Current unsupervised domain adaptation (UDA) methods for semantic segmentation typically assume identical class labels between the source and target domains. This assumption ignores the label-level domain gap, which is common in real-world scenarios, thus limiting their ability to identify finer-grained or novel categories without requiring extensive manual annotation. A promising direction to address this limitation lies in recent advancements in foundation models, which exhibit strong generalization abilities due to their rich prior knowledge. However, these models often struggle with domain-specific nuances and underrepresented fine-grained categories. To address these challenges, we introduce DynAlign, a framework that integrates UDA with foundation models to bridge both the image-level and label-level domain gaps. Our approach leverages prior semantic knowledge to align source categories with target categories that can be novel, more fine-grained, or named differently (e.g., vehicle to {car, truck, bus}). Foundation models are then employed for precise segmentation and category reassignment. To further enhance accuracy, we propose a knowledge fusion approach that dynamically adapts to varying scene contexts. DynAlign generates accurate predictions in a new target label space without requiring any manual annotations, allowing seamless adaptation to new taxonomies through either model retraining or direct inference. Experiments on the street scene semantic segmentation benchmarks GTA to Mapillary Vistas and GTA to IDD validate the effectiveness of our approach, achieving a significant improvement over existing methods. Our code will be publicly available.

==> rebuttal/clip_confidence.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table}[ht]
\centering
\caption{Ablations on CLIP confidence threshold
% Benchmarked on Mapillary and IDD following
% standard evaluation protocols on open-vocabulary model \cite{yu2024convolutions}.
}
\label{tab:clip_confidence}
%\setlength\tabcolsep{10pt}
\fontsize{8pt}{8pt}\selectfont
% \setlength{\tabcolsep}{3pt}
\setlength\extrarowheight{2.5pt}
\renewcommand{\arraystretch}{1.0}
%\resizebox{\textwidth}{!}{% 
\begin{tabular}{cc|cc|cc|cc|cc}
\toprule[1.5pt]
\multicolumn{2}{c|}{0.4} & \multicolumn{2}{c|}{0.5}  &\multicolumn{2}{c|}{0.6}   &\multicolumn{2}{c|}{0.7}  &\multicolumn{2}{c}{0.8}                          \\ 
 mACC & mIoU & mACC & mIoU & mACC & mIoU & mACC & mIoU & mACC & mIoU \\
% \Xhline{.5pt} 
\midrule
& & 53.0 & 36.7 & & & & & & \\
% \textcolor{blue}{HRDA} & & &? &? & & \\
% \textcolor{blue}{TACS?} & & &? &? & & \\
\bottomrule[1.5pt]

\end{tabular}
%}
\vspace{-0.5cm}
\end{table}

==> rebuttal/comparison_new.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table}[ht]
\centering
\caption{Open-vocabulary semantic segmentation comparisons on Mapillary Vistas and IDD
% Benchmarked on Mapillary and IDD following
% standard evaluation protocols on open-vocabulary model \cite{yu2024convolutions}.
}
\label{tab:result}
%\setlength\tabcolsep{10pt}
\fontsize{8pt}{8pt}\selectfont
% \setlength{\tabcolsep}{3pt}
\setlength\extrarowheight{2.5pt}
\renewcommand{\arraystretch}{1.0}
%\resizebox{\textwidth}{!}{% 
\begin{tabular}{c|c|cc|cc|cc}
\toprule[1.5pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Methods} & \multicolumn{2}{c}{all classes} & \multicolumn{2}{c}{known classes}  &\multicolumn{2}{c}{unknown classes}                           \\ \Xcline{3-8}{.5pt} 
& & mACC & mIoU & mACC & mIoU & mACC & mIoU \\
\Xhline{.5pt} 
\midrule
\multirow{5}{*}{Mapillary Vistas} 

& \textcolor{blue}{HRDA} & & &75.84 & 65.85 & & \\

& \textcolor{blue}{TACS?} & & &? &? & & \\

& Grounded-SAM & 33.1 & 28.6  & 46.7 & 43.0 & 24.0 & 18.3 \\
& OwlVIT-SAM  & 29.6 & 19.5 &  32.7 & 26.7 & 27.5 & 14.7 \\

\Xcline{2-8}{.5pt} 

& HRDA + Grounded-SAM & 40.4 &32.9 & 63.6 & 53.1 & 25.0 & 19.4 \\
& HRDA + OwlVIT-SAM& 40.2 & 28.8 & 56.1 & 48.4 & 29.5 & 15.6 \\
\Xcline{2-8}{.5pt} 
& Ours & \textbf{53.0}&\textbf{36.7} & \textbf{72.6} & \textbf{62.4} & \textbf{39.9} & \textbf{19.6} \\


\midrule
\midrule

& \textcolor{blue}{HRDA} & & &68.85 &61.34 & & \\

& \textcolor{blue}{TACS?} & & &? &? & & \\

\multirow{5}{*}{IDD} & Grounded-SAM  & 36.0 & 30.8 & 43.7 & 37.2 & 16.1 & 14.1 \\
& OwlVIT-SAM  & 31.6 & 20.9  &33.3 & 23.1 & 27.3 & 15.2\\

\Xcline{2-8}{.5pt} 

& HRDA + Grounded-SAM  & 51.7 &39.4 &65.6 & 49.3 & 16.1 & 14.1 \\
& HRDA + OwlVIT-SAM & 55.9 &40.2  & \textbf{67.1} & 49.9 & 27.3 & 15.2\\
% & Ours & 60.2 & 52.8 & 37.0 & 64.1 & 57.4 & 50.4 & 34.6& 40.2 & 34.1
\Xcline{2-8}{.5pt} 
% & Ours & 76.1 & \textbf{56.5} & \textbf{40.5} & 66.9 & \textbf{50.4} & \textbf{29.9} & 15.1 \\
% new mapping prob 0.6
% & Ours & 76.7 & \textbf{56.7} & \textbf{41.1} & 64.9 & \textbf{50.6} & \textbf{35.6} & \textbf{16.9} \\
% new mapping prob 0.7
% & Ours & 78.3 & \textbf{57.0} & \textbf{41.4} & 66.6 & \textbf{50.9} & \textbf{32.2} & \textbf{16.9} \\
% new mapping prob 0.7
& Ours & \textbf{57.7} & \textbf{41.7} & 66.8 & \textbf{50.9} & \textbf{34.3} & \textbf{18.1} \\
\bottomrule[1.5pt]

\end{tabular}
%}
\vspace{-0.5cm}
\end{table}

==> tables/ablations.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{wraptable}{r}{7.0cm}
% \begin{table}[H]
% \fontsize{8pt}{8pt}\selectfont
% \setlength{\tabcolsep}{8pt}
% \centering
% % \vspace{-0.5cm}
% \caption{Ablations on multi-scale visual feature and context-aware text feature}
% \label{tab:ablations}
% %\setlength\tabcolsep{15pt}
% \setlength\extrarowheight{2pt}
% \renewcommand{\arraystretch}{1.0}
% %\resizebox{\textwidth}{!}{% 
% \begin{tabular}{cc|cc|cc}
% \toprule[1.5pt]
%  \multicolumn{2}{c|}{Modules} & \multicolumn{2}{c}{Mapillary Vistas} & \multicolumn{2}{c}{IDD}  
%  % \vspace{0.1cm}
%  \\ \Xcline{3-6}{.5pt}
% MS (vision)  & CA (text) & mACC & mIoU & mACC & mIoU \\ 
% \cmidrule(l){1-6} 
% \XSolidBrush & \XSolidBrush & 44.0 & 29.0&52.9 & 37.9 \\
% \XSolidBrush & \Checkmark & 45.4 & 29.4&52.5 &38.0\\
% \Checkmark & \XSolidBrush & 50.2 & 35.6  & 57.0 & 39.9 \\
% \Checkmark & \Checkmark  & \textbf{53.0} & \textbf{36.7} & \textbf{57.7} & \textbf{41.7}
% % \midrule

% % 61.94 | 15.84 | 22.95  aAcc |  mIoU |  mAcc
 
% \\ \midrule
% \bottomrule[1.5pt]
% \end{tabular}
% \vspace{-0.5cm}
% \end{table}
% \end{wraptable}
\begin{table}[ht]
\centering
\caption{Ablations on multi-scale visual feature and context-aware text feature}
\label{tab:ablations}
\fontsize{8pt}{8pt}\selectfont
% \setlength{\tabcolsep}{15pt}
\setlength\extrarowheight{2pt}
%\setlength\tabcolsep{20pt}
\renewcommand{\arraystretch}{1.0}
%\resizebox{\textwidth}{!}{% 
\begin{tabular}{cc|cc|cc}
\toprule[1.5pt]
 \multicolumn{2}{c|}{Modules} & \multicolumn{2}{c}{Mapillary Vistas} & \multicolumn{2}{c}{IDD}  
 % \vspace{0.1cm}
 \\ \Xcline{3-6}{.5pt}
MS (vision)  & CA (text) & mACC & mIoU & mACC & mIoU \\ 
\cmidrule(l){1-6} 
\XSolidBrush & \XSolidBrush & 44.0 & 29.0&52.9 & 37.9 \\
\XSolidBrush & \Checkmark & 45.4 & 29.4&52.5 &38.0\\
\Checkmark & \XSolidBrush & 50.2 & 35.6  & 57.0 & 39.9 \\
\Checkmark & \Checkmark  & \textbf{53.0} & \textbf{36.7} & \textbf{57.7} & \textbf{41.7}
% \midrule

% 61.94 | 15.84 | 22.95  aAcc |  mIoU |  mAcc
 
\\ \midrule
\bottomrule[1.5pt]
\end{tabular}
\end{table}


==> tables/clip_ablations.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{wraptable}{r}{7.0cm}
% \centering
% \vspace{-0.5cm}
\caption{Ablation study: comparing CLIP vision encoders as backbone networks}
\label{tab:clip_ablations}
\fontsize{8pt}{8pt}\selectfont
% \setlength{\tabcolsep}{15pt}
\setlength\extrarowheight{2pt}
%\setlength\tabcolsep{20pt}
\renewcommand{\arraystretch}{1.0}
%\resizebox{\textwidth}{!}{% 
\begin{tabular}{c|cc|cc}
\toprule[1.5pt]
\multirow{2}{*}{model} & \multicolumn{2}{c}{Mapillary Vistas} & \multicolumn{2}{c}{IDD} \vspace{0.05cm} \\ 
\Xcline{2-5}{.5pt}
\vspace{0.05cm}
 & mACC & mIoU  & mACC & mIoU \\
\midrule
CLIP & 50.8 & 35.0 & 54.7 & 38.0 \\
MaskCLIP  & 50.5 & 34.7 & 54.1 & 37.5\\
SCLIP & 50.9 & 36.0 & 56.8  & 39.4\\
ConvCLIP & \textbf{53.0}&\textbf{36.7} & \textbf{57.7} & \textbf{41.7} \\
\bottomrule[1.5pt]
\end{tabular}
\end{wraptable}

==> tables/comparison_with_sota.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table}[ht]
\centering
\caption{Comparison with SOTA methods}
\label{tab:unsupervised}
\setlength\tabcolsep{5pt}
\renewcommand{\arraystretch}{1.0}
\resizebox{\textwidth}{!}{% 
\begin{tabular}{c|c|ccc|ccc|ccc}
\toprule[1.5pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{all classes} & \multicolumn{3}{c}{known classes}  &\multicolumn{3}{c}{unknown classes}                           \\ \cmidrule(l){3-11} 
& & aACC & mACC & mIoU & aAcc & mACC & mIoU & aAcc & mACC & mIoU\\
\midrule
\multirow{3}{*}{Mapillary} 

& Grounded-SAM & 69.3 & 33.1 & 28.6   & 72.8 & 45.8 & 43.2 & 19.7 & 24.0 & 22.0 \\
& OwlVIT-SAM & 49.6 & 29.6 & 19.5 &  51.1 & 33.0 & 27.3 & 27.8 & 27.5 & 22.7 \\
& Ours & 82.1 & 53.0&36.7 & 84.8& 70.0 & 62.3 & 42.4 & 39.9 & 30.0 \\


\midrule

\multirow{3}{*}{IDD} & Grounded-SAM  & 58.7 & 36.0 & 30.8 & 65.1 & 43.7 & 38.9 & 14.4 & 16.1 & 15.4 \\
& OwlVIT-SAM & 53.1 & 31.6 & 20.9  & 59.0 & 33.3 & 24.4 & 12.1 & 27.3 & 18.6\\
% & Ours & 60.2 & 52.8 & 37.0 & 64.1 & 57.4 & 50.4 & 34.6& 40.2 & 34.1
& Ours & 76.1 & 56.5 & 40.5 & 84.3 & 66.9 & 57.7 & 19.1 & 29.9 & 26.7
% mapi  mIoU,fwIoU,mACC,pACC 31.8105,70.0254,42.7307,79.2851
\\ \midrule
\bottomrule[1.5pt]
\end{tabular}
}
\end{table}

==> tables/da_comparison.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table}[H]
\centering
\caption{Comparison under DA}
\label{tab:da}
\setlength\tabcolsep{5pt}
\renewcommand{\arraystretch}{1.0}
\resizebox{\textwidth}{!}{% 
\begin{tabular}{c|c|ccc|ccc|ccc}
\toprule[1.5pt]
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{all classes} & \multicolumn{3}{c}{known classes}  &\multicolumn{3}{c}{unknown classes}                           \\ \cmidrule(l){3-11} 
& & aACC & mACC & mIoU & aAcc & mACC & mIoU & aAcc & mACC & mIoU\\
\midrule
\multirow{3}{*}{Mapillary} 

& HRDA + Grounded-SAM & 84.9&40.4 &32.9 & 89.5 & 61.7 & 53.9 & 19.9 & 25.0 & 22.7 \\
& HRDA + OwlVIT-SAM & 68.1 & 40.2 & 28.8 & 70.9 & 55.1 & 48.5 & 28.1 & 29.5 & 23.9 \\
& Ours & 82.1 & 53.0&36.7 & 84.8& 70.0 & 62.3 & 42.4 & 39.9 & 30.0 \\


\midrule

\multirow{3}{*}{IDD} 
& HRDA + Grounded-SAM  & 80.6 & 51.7 &39.4 &90.1 &65.6 &56.1 &14.4 &16.1 &15.4 \\
& HRDA + OwlVIT-SAM & 80.3 & 55.9 &40.2  & 90.1 & 63.6 &51.7&12.1 &27.3 &18.6\\
% & Ours & 60.2 & 52.8 & 37.0 & 64.1 & 57.4 & 50.4 & 34.6& 40.2 & 34.1
& Ours & 76.1 & 56.5 & 40.5 & 84.3 & 66.9 & 57.7 & 19.1 & 29.9 & 26.7
% mapi  mIoU,fwIoU,mACC,pACC 31.8105,70.0254,42.7307,79.2851
\\ \midrule
\bottomrule[1.5pt]
\end{tabular}
}
\end{table}
